Codebook Based Two-Time Scale Resource Allocation Design for IRS-Assisted eMBB-URLLC Systems

This paper investigates the resource allocation algorithm design for wireless systems assisted by large intelligent reflecting surfaces (IRSs) with coexisting enhanced mobile broadband (eMBB) and ultra reliable low-latency communication (URLLC) users. We consider a two-time scale resource allocation scheme, whereby the base station's precoders are optimized in each mini-slot to adapt to newly arriving URLLC traffic, whereas the IRS phase shifts are reconfigured only in each time slot to avoid excessive base station-IRS signaling. To facilitate efficient resource allocation design for large IRSs, we employ a codebook-based optimization framework, where the IRS is divided into several tiles and the phase-shift elements of each tile are selected from a pre-defined codebook. The resource allocation algorithm design is formulated as an optimization problem for the maximization of the average sum data rate of the eMBB users over a time slot while guaranteeing the quality-of-service (QoS) of each URLLC user in each mini-slot. An iterative algorithm based on alternating optimization (AO) is proposed to find a high-quality suboptimal solution. As a case study, the proposed algorithm is applied in an industrial indoor environment modelled via the Quadriga channel simulator. Our simulation results show that the proposed algorithm design enables the coexistence of eMBB and URLLC users and yields large performance gains compared to three baseline schemes. Furthermore, our simulation results reveal that the proposed two-time scale resource allocation design incurs only a small performance loss compared to the case when the IRSs are optimized in each mini-slot.

==> Fig1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA Number of URLLC users data bits, $B_{j,\textrm{req}}$}%
\psfrag{010}[bc][bc]{\matlabtextA Average sum data rate for eMBB users (bits/s/Hz)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $150$}%
\psfrag{001}[ct][ct]{\matlabtextB $200$}%
\psfrag{002}[ct][ct]{\matlabtextB $250$}%
\psfrag{003}[ct][ct]{\matlabtextB $300$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $5$}%
\psfrag{006}[rc][rc]{\matlabtextB $10$}%
\psfrag{007}[rc][rc]{\matlabtextB $15$}%
\psfrag{008}[rc][rc]{\matlabtextB $20$}%
%
%% </ytick>

==> Fig2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA Maximum transmit power of the BS [dBm]}%
\psfrag{011}[bc][bc]{\matlabtextA Average sum data rate for eMBB users (bits/s/Hz)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $25$}%
\psfrag{001}[ct][ct]{\matlabtextB $30$}%
\psfrag{002}[ct][ct]{\matlabtextB $35$}%
\psfrag{003}[ct][ct]{\matlabtextB $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $5$}%
\psfrag{006}[rc][rc]{\matlabtextB $10$}%
\psfrag{007}[rc][rc]{\matlabtextB $15$}%
\psfrag{008}[rc][rc]{\matlabtextB $20$}%
\psfrag{009}[rc][rc]{\matlabtextB $25$}%
%
%% </ytick>
